Measurement-Robust Control Barrier Functions: Certainty in Safety with Uncertainty in State

The increasing complexity of modern robotic systems and the environments they operate in necessitates the formal consideration of safety in the presence of imperfect measurements. In this paper we propose a rigorous framework for safety-critical control of systems with erroneous state estimates. We develop this framework by leveraging Control Barrier Functions (CBFs) and unifying the method of Backup Sets for synthesizing control invariant sets with robustness requirements -- the end result is the synthesis of Measurement-Robust Control Barrier Functions (MR-CBFs). This provides theoretical guarantees on safe behavior in the presence of imperfect measurements and improved robustness over standard CBF approaches. We demonstrate the efficacy of this framework both in simulation and experimentally on a Segway platform using an onboard stereo-vision camera for state estimation.

==> IncrementalStability.tex <==

The forward integration of a non-singleton set required to evaluate this condition presents a computational problem. To overcome this, we introduce the concept of incremental stability which allows us to simply forward integrate our state estimate $\widehat{\mb{x}}$. 

\begin{definition}(Incremental Stability \cite{angeli2002Lyapunov})
    The dynamical system in \eqref{eq:dynamics} is incrementally stable inside a set $\mathcal{X} \subseteq \R^n$ if $\forallT \geq 0 $, $\forall \mb{x}_1, \mb{x}_2 \in \mathcal{X}$ and $\mb{k}: [0,T] \to \R^m $ such that $\phi_t^\mb{k}(\mb{x}_1)$ and $\phi_t^{\mb{k}}(\mb{x}_2)$ stay inside $\mathcal{X}$, the evolution of the state satisfies $\Vert \phi_t^{\mb{k}}(\mb{x}_1) - \phi_t^{\mb{k}}(\mb{x}_2)  \Vert \leq \beta(\Vert \mb{x}_1 - \mb{x}_2 \Vert, t )$, where $\beta: \R\times [0, T] \to \R $ is non-increasing $t$ and $\forall t \in [0, T], \beta (\cdot, t) $ is a class-$\mathcal{K}$ function. 
\end{definition}

Assuming incremental stability of our system, we have the following set relation: 
\begin{equation}
\mathcal{R}(\widehat{\mb{x}} \oplus - \mathcal{E}(\mb{y}), \Delta t) \subseteq \mathcal{R}(\widehat{\mb{x}}) \oplus - \mathcal{E}(\mb{y}). 
\end{equation}
Thus, for an incrementally stable sampled-data system with a zero-order hold controller and measurement-model error, enforcing the robustified safety conditions: 
\begin{align}
    \inf_{\mb{z} \in \mathcal{R}(\widehat{\mb{x}} , \Delta t)- \mathcal{E}(\mb{y})}   \quad \derp{h}{\mb{x}}\bigg\rvert_{\phi_\tau^{\overline{\mb{k}}_B}(\mb{z})} \derp{\phi_t^{\overline{\mb{k}}_B}}{\mb{x}}\bigg\rvert_{\mb{z}}\bigg( \mb{f}(\mb{z}) + \mb{g}(\mb{z})\mb{u}  \bigg) \geq -\alpha_\tau (h_\tau (\mb{x})), \nonumber\\
    \inf_{\mb{z} \in \mathcal{R}(\widehat{\mb{x}}, \Delta t)- \mathcal{E}(\mb{y})} \quad \derp{h_B}{\mb{x}}\bigg\rvert_{\phi_T^{\overline{\mb{k}}_B}(\mb{z})} \derp{\phi_t^{\overline{\mb{k}}_B}}{\mb{x}}\bigg\rvert_{\mb{z}}\bigg( \mb{f}(\mb{z}) + \mb{g}(\mb{z})\mb{u}  \bigg) \geq -\alpha_B(h_B(\mb{x})) \label{eq:backup_set_const_SDS_state_estimate}
\end{align}
for all time $\tau \in [t, t + T] $ is sufficient for to render to the system safe with respect to $\overline{\mathcal{C}_I}$. We have the following lemma relating the constraints in \eqref{eq:backup_set_const_SDS_state_estimate} and the safety of $\overline{\mathcal{C}_I}$:
\begin{lemma}[\cite{singletary2020control}]
    Let $\overline{u}_i$ be an input signal with zero-order hold that satisfies \eqref{eq:backup_set_const_SDS}. If the system is incrementally stable in $\overline{\mathcal{C}_I}$, then the system is safe with respect to $\overline{\mathcal{C}_I}$. \label{lm:sds}
\end{lemma}

==> ZoH.tex <==

\hl{introduce SDS zero order hold} 



While condition \eqref{eq:backup_set_const} can be used to guarantee safety for continuous-time systems, it relies on the input being continuous. In the presence of a zero-order hold control implementation nearly ubiquitous in sampled-data systems, the description of the invariant set needs to be modified. The zero-order hold backup controller, denoted as $\overline{\mb{k}}_B(x(\cdot), t)$, simply takes on the value of $\mb{k}_B (x)$ every $\Delta t$ seconds, and holds that value until its next update:
\begin{equation}
    \overline{\mb{k}}_B(x(\cdot), t) = \mb{k}_B\left(x\left(\left\lfloor \frac{t}{\Delta_t}\right\rfloor\Delta t\right)\right) , 
\end{equation}
where $\left\lfloor \cdot \right\rfloor$ is the largest integer not greater than the argument.
\begin{remark}
The flow of the system under the zero-order backup controller $\phi^{\overline{\mb{k}}_B}_t(x)$ is well-defined, as unique solutions to sampled-data systems exist so long as the underlying controller is piecewise continuous (c.f. [19, p. 16])
\end{remark}
The updated control invariant set under the zero-order holdbackup controller can be written as
\begin{equation}
    \overline{\mathcal{C}_I } = \left\{\begin{array}{l|c}
        & h(\phi_\tau^{\overline{\mb{k}}_B}) \geq 0, \forall \tau \in [0, T ]\\
        \mb{x} \in \mathcal{X} &  \textrm{and} \\
        &  h_B(\phi_T^{\overline{\mb{k}}_B}) \geq 0 
        \end{array}\right\}.
\end{equation}
This is a control invariant set for the system under a zero-order controller $\overline{\mb{k}}_B$. The proof follows from \cite[Theorem 1]{gurriet2018online}.

\hl{Backup set approach for ZoH controller.}

In limiting ourselves to zero-order hold controllers, it follows that the conditions \eqref{eq:backup_set_const} must be met over the entire time horizon of the zero-order hold controller. Note that this consideration must be taken regardless of the method used for expressing the robust control barrier function, and was a subject of prior research of the authors \cite{gurriet2019realizable}. \textcolor{blue}{ < - - check this}

To express this precisely, we consider the set $\mathcal{R}(\mb{x}, \Delta t) \subset \mathcal{X}$,  the set of reachable states from point $\mb{x}$ in time $\Delta t $. %, and the set $\mathcal{E}(\mb{y}) $ to be the measurement uncertainty set for some measurement $\mb{y}$. 
Using this definition, enforcing the constraints:
% \begin{equation}
%     h(\mathcal{R}(\mb{x}_0)) \geq 0 \implies h( \phi_\tau^{\overline{\mb{k}}_B}(\mb{x}_0)) \geq 0, \; \; \forall \tau \in [0, \Delta_t]
% \end{equation}
\begin{align}
    \inf_{\mb{z} \in \mathcal{R}(\mb{x}) , \Delta t)}   \quad \derp{h}{\mb{x}}\bigg\rvert_{\phi_\tau^{\overline{\mb{k}}_B}(\mb{z})} \derp{\phi_t^{\overline{\mb{k}}_B}}{\mb{x}}\bigg\rvert_{\mb{z}}\bigg( \mb{f}(\mb{z}) + \mb{g}(\mb{z})\mb{u}  \bigg) \geq -\alpha_\tau(h_\tau(\mb{x})), \nonumber\\
    \inf_{\mb{z} \in \mathcal{R}(\mb{x}), \Delta t)} \quad \derp{h_B}{\mb{x}}\bigg\rvert_{\phi_T^{\overline{\mb{k}}_B}(\mb{z})} \derp{\phi_t^{\overline{\mb{k}}_B}}{\mb{x}}\bigg\rvert_{\mb{z}}\bigg( \mb{f}(\mb{z}) + \mb{g}(\mb{z})\mb{u}  \bigg) \geq -\alpha_B(h_B(\mb{x}))   \label{eq:backup_set_const_SDS}
\end{align}
at each update of the zero-order hold controller, renders the system safe with respect to $\overline{\mathcal{C}_I}$ for all time $t\geq 0$. 

==> notes.tex <==
\section{NOTES}

\newpage
Verifying that this condition holds can be difficult for an arbitrary CBF, and it is not easily (or possibly) enforced in a convex-optimization based controller. To resolve these problems, the following definition was introduced:



\hl{MRCBF Definition}

\begin{definition}[\textit{Measurement-Robust Control Barrier Function (MR-CBF) \cite{dean2020guaranteeing}}]
Let $\C\subset\R^n$ be the 0-superlevel set of a continuously differentiable function $h:\R^n\to\R$ with $0$ a regular value. The function $h$ is a \textit{Measurement-Robust Control Barrier Function} (MR-CBF) for \eqref{eq:dynamics} on $\C$ with \textit{parameter function} $(a,b):\R^k\to\R^2_+$ if there exists $\alpha\in \mathcal{K}_{\infty,e}$ such that for all $(\mb{y},\widehat{\mb{x}})\in\widehat{\mb{v}}(\C)$:
\begin{equation}
\label{eqn:mr-cbf}
     \sup_{\mb{u}\in\R^m} L_\mb{f}h(\widehat{\mb{x}})+L_\mb{g}h(\widehat{\mb{x}})\mb{u} - (a(\mb{y}) + b(\mb{y}) \Vert\mb{u}\Vert_2)  >-\alpha(h(\widehat{\mb{x}})).
\end{equation}
\end{definition}
%Verifying this condition over $\widehat{\mb{v}}(\C)$ may not be possible, but as will be seen in Section \ref{sec:learning},  the set $\widehat{\mathcal{X}}(\mb x)$ can be used to provide sufficient conditions under which~\eqref{eqn:mr-cbf} is met. 
%The definition of a MR-CBF introduces the non-positive term $-(a(\mb{y})+b(\mb{y})\Vert\mb{u}\Vert_2)$ to the control barrier condition, requiring that a stronger degree of safety be enforced compared to the typical CBF condition \eqref{eq:cbf_constraint}. Furthermore, the norm of the input appears in this term, indicating that for large values of $b$ large inputs can lead to unsafe behavior. This condition is equivalently stated as:
% \begin{equation}
% \label{eqn:mrcbfalt}
%     \Vert L_\mb{g}h(\widehat{\mb{x}}) \Vert_2 \leq b(\mb{y}) \implies L_\mb{f}h(\widehat{\mb{x}}) > -\alpha(h(\widehat{\mb{x}})) + a(\mb{y}). 
% \end{equation}
% In contrast to the implication in \eqref{eqn:cbfalt}, the size of set for which the antecedent in \eqref{eqn:mrcbfalt} is met may be larger, requiring the natural dynamics to be safe ($L_\mb{f}h(\widehat{\mb{x}}) > -\alpha(h(\widehat{\mb{x}})) + a(\mb{y})$) in a larger region. Given a MR-CBF $h$ for \eqref{eqn:eom} on $\C$ with parameter function $(a,b)$ and a corresponding $\alpha\in\cal{K}_{\infty,e}$, we can consider the pointwise set of all control values that satisfy \eqref{eqn:mr-cbf}:
\begin{align}
\label{eqn:Kmrcbf}
    K_{\textrm{mr-cbf}}(\mb{y},\widehat{\mb{x}})  & \triangleq \nonumber \\
    \Bigg\{
    \mb{u}\in\R^m  \;&  \begin{array}{|rl}
         L_\mb{f}h(\widehat{\mb{x}})+L_\mb{g}h(\widehat{\mb{x}})\mb{u} & - ( a(\mb{y}) + b(\mb{y}) \Vert\mb{u}\Vert_2)\\
         & \geq -\alpha(h(\widehat{\mb{x}})) 
    \end{array} \Bigg\}
\end{align}
for $(\mb{y},\widehat{\mb{x}})\in\widehat{\mb{v}}(\C)$. Given this construction, we have the following result relating the existence of a MR-CBF to safety under the presence of measurement model uncertainty:

\hl{MRCBF Theorem}

\begin{theorem}\label{thm:safety}
Let a set $\C\subset\R^n$ be defined as the 0-superlevel set of a continuously differentiable function $h:\R^n\to\R$. Assume the functions $L_\mb{f}h:\R^n\to\R$, $L_\mb{g}h:\R^n\to\R^m$, and $\alpha\circ h:\R^n\to\R$ are Lipschitz continuous on $\C$ with Lipschitz coefficients $\mathfrak{L}_{L_\mb{f}h}$, $\mathfrak{L}_{L_\mb{g}h}$, and $\mathfrak{L}_{\alpha\circ h}$, respectively. Further assume there exists a locally Lipschitz function $\epsilon:\R^k\to\R_+$, such that $\max_{\mb{e}\in\mathcal{E}(\mb{y})}\Vert\mb{e}\Vert_2\leq\epsilon(\mb{y})$ for all $\mb{y} \in \mb{p}(\C)$. If $h$ is a MR-CBF for \eqref{eq:dynamics} on $\C$ with parameter function $(\epsilon(\mb{y})(\mathfrak{L}_{L_\mb{f}h}+\mathfrak{L}_{\alpha\circ h}),\epsilon(\mb{y})\mathfrak{L}_{L_\mb{g}h})$, then any locally Lipschitz continuous controller $\mb{k}:\R^k\times\R^n\to\R^m$, such that $\mb{k}(\mb{y},\widehat{\mb{x}})\in K_{\textrm{mr-cbf}}(\mb{y},\widehat{\mb{x}})$ for all $(\mb{y},\widehat{\mb{x}})\in\widehat{\mb{v}}(\C)$, renders the system \eqref{eqn:cloop} safe w.r.t. $\C$.
\end{theorem}
% \begin{proof}
% See Appendix \ref{app:mrcbfproof} in the supplementary material for this paper.
% \end{proof}

A proof of this theorem can be found in Appendix \ref{app:mrcbfproof}. To more clearly see how the upper bound on the estimate error, $\epsilon(\mb{y})$, manifests in the MR-CBF condition, we note the particular condition that must be satisfied for this theorem is given by:
\begin{equation}
    \label{eqn:mrcbflip}
     \sup_{\mb{u}\in\R^m} L_\mb{f}h(\widehat{\mb{x}})+L_\mb{g}h(\widehat{\mb{x}})\mb{u}-\epsilon(\mb{y})(\mathfrak{L}_{L_\mb{f}h}+\mathfrak{L}_{\alpha\circ h}+\mathfrak{L}_{L_\mb{g}h}\Vert\mb{u}\Vert_2)>-\alpha(h(\widehat{\mb{x}})).
\end{equation}
%Thus as $\epsilon(\mb{y})$ becomes smaller, the level of robustness required by an MR-CBF approaches that of a regular CBF for the same set $\C$, and recovers the original control barrier condition with no estimate error. Furthermore, smaller values of $\epsilon(\mb{y})$ can be interpreted as leading to an enlarging of the region over which the condition \eqref{eqn:mrcbfalt} holds.

% WE DONT ACTUALLY NEED THE MRCBF FILTER SINCE WE"RE GOING TO USE A DIFFERENT FILTER
% One advantage of this approach for resolving the impact of measurement model uncertainty on safety is that the constraint in \eqref{eqn:Kmrcbf} remains convex. This constraint can then be directly integrated into an optimization based controller as follows:
% \begin{align}
% \label{eqn:MR-OP}
% \tag{MR-OP}
% \mb{k}(\mb{y},\widehat{\mb{x}}) =  \,\,\underset{\mb{u} \in \R^m}{\argmin}  &  \quad \frac{1}{2} \Vert \mb{u}-\mb{k}_d(\widehat{\mb{x}}) \Vert_2^2  \\
% %\tag{CLF}
% \mathrm{s.t.} \quad & \quad L_\mb{f}h(\widehat{\mb{x}})-(\mathfrak{L}_{L_\mb{f}h}+\mathfrak{L}_{\alpha\circ h})\epsilon(\mb{y})+L_\mb{g}h(\widehat{\mb{x}})\mb{u}-\mathfrak{L}_{L_\mb{g}h}\epsilon(\mb{y})\Vert\mb{u}\Vert_2\geq-\alpha(h(\widehat{\mb{x}})). \nonumber
% \end{align}
%This problem is in fact a second-order cone program (SOCP), with an explicit conversion to standard form provided in Appendix \ref{app:mropsocp}. As this constraint is non-smooth, existing methods for computing closed-form solutions via Lagrangian duality and assessing Lipschitz continuity \cite{jankovic2018robust} are not applicable. Future work will consider methods from variational analysis to study the Lipschitz continuity of solutions to this problem \cite{mordukhovich2014full}. In practice, a slack variable, $\delta$, is often added to ensure constraint feasibility. This relaxation is penalized in the cost with a large coefficient $p\in\R_{++}$:
%\begin{align}
%\label{eqn:R-MR-OP}
% \tag{R-MR-OP}
% \mb{k}(\mb{y},\widehat{\mb{x}}) =  \,\,\underset{(\mb{u},\delta) \in \R^m\times\R}{\argmin}  &  \quad \frac{1}{2} \Vert \mb{u}-\mb{k}_d(\widehat{\mb{x}}) \Vert_2^2 + p\delta^2  \\
% %\tag{CLF}
% \mathrm{s.t.} \quad   L_\mb{f}h&(\widehat{\mb{x}})-(\mathfrak{L}_{L_\mb{f}h}+\mathfrak{L}_{\alpha\circ h})\epsilon(\mb{y})+L_\mb{g}h(\widehat{\mb{x}})\mb{u}-\mathfrak{L}_{L_\mb{g}h}\epsilon(\mb{y})\Vert\mb{u}\Vert_2\geq-\alpha(h(\widehat{\mb{x}}))-\delta. \nonumber
% \end{align}


%While this relaxed controller does not necessarily enforce the desired safety constraint, if $\delta$ remains small the impact on safety can be understood through the notion of projection-to-state safety \cite{taylor2020control}. Furthermore, this relaxation ensures that the resulting controller is locally Lipschitz continuous as made explicit in Appendix \ref{app:rmroplipschitz} via the methods in \cite{dontchev1993lipschitzian}.

\subsection{$m$-inequality}
Consider some continuously differentiable function $f$, points $\widehat{\mb{x}} +\mb{e}$ and $\widehat{\mb{x}}$, and a function $g(s) = f(s(\widehat{\mb{x}} +\mb{e}) + (1-s)\widehat{\mb{x}})$.
\begin{align}
    ||f(\widehat{\mb{x}} +\mb{e}) - f(\widehat{\mb{x}})|| & = ||g(1) - g(0) || \\
    & = ||\int_0^1 \frac{dg}{ds}(s) ds || \\
    & = \| \int_0^1 Df(s(\widehat{\mb{x}} +\mb{e}) + (1-s)\widehat{\mb{x}})ds (s(\widehat{\mb{x}} +\mb{e}) + (1-s)\widehat{\mb{x}}) \| \\
    & \leq \int_0^1 \|Df(s(\widehat{\mb{x}} +\mb{e}) + (1-s)\widehat{\mb{x}})\|ds \|s(\widehat{\mb{x}} +\mb{e}) + (1-s)\widehat{\mb{x}}\| 
\end{align}
$\overline{\mathcal{B}_{\epsilon(\mb{y})}(\widehat{\mb{x}})}\cap \textrm{span}\{B\}$ is the intersection of two convex sets so it is convex and contains $(s(\widehat{\mb{x}} +\mb{e}) + (1-s)\widehat{\mb{x}})$ for all $s \in [0,1]$. By maximizing the integrand over $\overline{\mathcal{B}_{\epsilon(\mb{y})}(\widehat{\mb{x}})}\cap \textrm{span}\{B\}$ we recover $m(f, \mb{y}, \widehat{\mb{x}})$. By also bounding the error, the bound on $||f(\widehat{\mb{x}} +\mb{e}) - f(\widehat{\mb{x}})||$ becomes: 
\begin{align}
    ||f(\widehat{\mb{x}} +\mb{e}) - f(\widehat{\mb{x}})|| & \leq m(f, \mb{y}, \widehat{\mb{x}})\epsilon(\mb{y})
\end{align}

